Low-Resolution Horizontal and Vertical Layered Mutual Information Maximizing LDPC Decoding

We investigate iterative low-resolution message-passing algorithms for quasi-cyclic LDPC codes with horizontal and vertical layered schedules. Coarse quantization and layered scheduling are highly relevant for hardware implementations to reduce the bit width of messages and the number of decoding iterations. As a novelty, this paper compares the two scheduling variants in combination with mutual information maximizing compression operations in variable and check nodes. We evaluate the complexity and error rate performance for various configurations. Dedicated hardware architectures for regular quasi-cyclic LDPC decoders are derived on a conceptual level. The hardware-resource estimates confirm that most of the complexity lies within the routing network operations. Our simulations reveal similar error rate performance for both layered schedules but a slightly lower average iteration count for the horizontal decoder.

==> other.tex <==
%auto-ignore



\begin{itemize}
	\item OMSQ requires 6 bits vor $y^v$ message and routing networks can be organized such that one permutation with 6 bits replaces 2 permutations with 3 bits.
	\item OMSQ requires offset operation adding delay
	\item OMSQ requires 4-bit comparisons if range is -8 to +7. 3-bit comparisons are required if range is limited to -7 to +7. On the other hand, the 3-bit decoding requires 2-bit comparators which decreases delay by 33 percent.
	\item IB requires translation stage here 2 bits are mapped to 6 bits, which adds similar delay as the offset operation.
	\item IB requires 8-bit adder unit which adds two full adder delays if ripple carry is used, increasing delay by 8/6=33 percent.
	\item Per layer update only one addition contributes to the decoder delay, but $\log_2(d_c)$ comparisons add delay at the check node when using a tree structure. Overall less decoding delay can be achieved, however at the price of a 0.02 dB performance loss.
	\item The average number of iterations might be significantly higher for 3-bit decoding. However, this requires a syndrome check which is not always done in practice. Checking the syndrome require additional complexity since all information must be merged with and-gate operations. E.g. for $M$ check node a tree structure add $log_2(M)$ delays of and-gates. If $M=2048=K(1/R-1)$ we would have 11 and-gate delays. 
	\item In layered decoding the memory consumption for $t^c$ messages is reduced from 4 to 3 bits. However, the memory consumption for $y^{v}$ increased from 6 to 8 (not really memory because it is reused in consecutive layers)
\end{itemize}
\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{ber_rate_1_2_4bit}
	\caption{}
	\label{fig:_berrate124bit}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{ber_rate_5_6_4bit}
	\caption{}
	\label{fig:_berrate564bit}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{ber_rate_5_6_2to4bit}
	\caption{}
	\label{fig:_berrate562to4bit}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{avg_iter_rate_5_6_2to4bit1}
	\caption{}
	\label{fig:_avgiterrate562to4bit1}
\end{figure}
\section{Complexity Analysis}
Exploit isomorphic structure for barrel shifter complexity savings.
\subsection{Barrel Shifter (Transistor Count)}
\cite{boutillon_extended_2020}
\subsection{Relevance of Coarsely Quantized Message Passing Compared to Node Complexity}
\subsection{Memory Complexity}
\subsection{Discussion}
\begin{itemize}
	\item Vertical decoder requires less area for maximum parallel implementation. Does memory or computation require higher complexity?
	\item More efficient if time between memory updates is small. Otherwise memory just takes chip area without usage. The time is reduced by passing less bits between CN and VN.
	\item CH memory is just read only memory in vertical decoder during decoding.
	\item Precompute sum of VN while performing CN update. This minimizes the decoding delay significantly, in best case to a single summation to obtain the next VTC message.
	\item To decrease the delay, one could use very fast adder for the critical path, but more efficient higher delay adders for the precomputation.
\end{itemize}



==> standalones/avg_iterations_min_comp_uni_44_43_42/data.tex <==

\addplot [semithick, red!75.2941176470588!black, mark=square*, mark size=1.75, mark options={solid}]
table {%
1 10
1.1 10
1.2 10
1.3 10
1.4 10
1.5 10
1.6 10
1.7 10
1.8 10
1.9 10
2 10
2.1 10
2.2 10
2.3 10
2.4 10
2.5 10
2.6 10
2.7 9.999
2.8 9.974
2.9 9.9
3 9.42
3.1 8.422
3.2 6.946
3.3 5.60028571428571
3.4 4.5725
3.5 3.86715
3.6 3.3512380952381
3.7 2.95511363636364
3.8 2.61286666666667
3.9 2.33639130434783
4 2.12663829787234
4.1 1.95385106382979
4.2 1.786
4.3 1.60218
4.4 1.41464705882353
4.5 1.25796153846154
4.6 1.15069811320755
4.7 1.07656603773585
4.8 1.03362264150943
4.9 1.00915094339623
};
\addplot [semithick, red!75.2941176470588!black, dotted, mark=triangle*, mark size=2.5, mark options={solid}]
table {%
1 10
1.1 10
1.2 10
1.3 10
1.4 10
1.5 10
1.6 10
1.7 10
1.8 10
1.9 10
2 10
2.1 10
2.2 10
2.3 10
2.4 10
2.5 10
2.6 10
2.7 10
2.8 9.996
2.9 9.979
3 9.817
3.1 9.314
3.2 8.175
3.3 6.682
3.4 5.38466666666667
3.5 4.47728205128205
3.6 3.82239024390244
3.7 3.35
3.8 2.95318181818182
3.9 2.63093333333333
4 2.36067391304348
4.1 2.14829787234043
4.2 1.974875
4.3 1.80334693877551
4.4 1.61834
4.5 1.43543137254902
4.6 1.28384615384615
4.7 1.16692452830189
4.8 1.09120754716981
4.9 1.04362264150943
};
\addplot [semithick, red!75.2941176470588!black, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=x, mark size=2.5, mark options={solid}]
table {%
1 10
1.1 10
1.2 10
1.3 10
1.4 10
1.5 10
1.6 10
1.7 10
1.8 10
1.9 10
2 10
2.1 10
2.2 10
2.3 10
2.4 10
2.5 10
2.6 10
2.7 10
2.8 10
2.9 9.999
3 10
3.1 9.984
3.2 9.84
3.3 9.337
3.4 8.326
3.5 6.92466666666667
3.6 5.7423
3.7 4.86835897435897
3.8 4.21075609756097
3.9 3.71267441860465
4 3.298
4.1 2.93709090909091
4.2 2.63536170212766
4.3 2.37079166666667
4.4 2.15122448979592
4.5 1.94036
4.6 1.74882352941176
4.7 1.55943396226415
4.8 1.39996226415094
4.9 1.26898148148148
};
\addplot [semithick, color0, mark=square*, mark size=1.75, mark options={solid}]
table {%
1 10
1.1 10
1.2 10
1.3 10
1.4 10
1.5 10
1.6 10
1.7 10
1.8 10
1.9 10
2 10
2.1 10
2.2 10
2.3 10
2.4 10
2.5 10
2.6 10
2.7 9.999
2.8 9.982
2.9 9.929
3 9.569
3.1 8.697
3.2 7.3295
3.3 6.03083333333333
3.4 5.00205714285714
3.5 4.28308108108108
3.6 3.7605
3.7 3.35879487179487
3.8 3.01830952380952
3.9 2.73604651162791
4 2.49163636363636
4.1 2.29056818181818
4.2 2.12835555555556
4.3 1.99468888888889
4.4 1.86889130434783
4.5 1.73327659574468
4.6 1.58968085106383
4.7 1.44404081632653
4.8 1.31659183673469
4.9 1.21694
};
\addplot [semithick, color0, dotted, mark=triangle*, mark size=2.5, mark options={solid}]
table {%
1 10
1.1 10
1.2 10
1.3 10
1.4 10
1.5 10
1.6 10
1.7 10
1.8 10
1.9 10
2 10
2.1 10
2.2 10
2.3 10
2.4 10
2.5 10
2.6 10
2.7 10
2.8 9.995
2.9 9.983
3 9.865
3.1 9.389
3.2 8.389
3.3 7.095
3.4 5.8045
3.5 4.91877777777778
3.6 4.27163157894737
3.7 3.77741025641026
3.8 3.36546341463415
3.9 3.03717073170732
4 2.74881395348837
4.1 2.49438636363636
4.2 2.28853333333333
4.3 2.12584782608696
4.4 1.98242553191489
4.5 1.84446808510638
4.6 1.70142553191489
4.7 1.5515306122449
4.8 1.41544897959184
4.9 1.29618
};
\addplot [semithick, color0, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=x, mark size=2.5, mark options={solid}]
table {%
1 10
1.1 10
1.2 10
1.3 10
1.4 10
1.5 10
1.6 10
1.7 10
1.8 10
1.9 10
2 10
2.1 10
2.2 10
2.3 10
2.4 10
2.5 10
2.6 10
2.7 10
2.8 10
2.9 10
3 10
3.1 9.987
3.2 9.893
3.3 9.53
3.4 8.652
3.5 7.34
3.6 6.20214285714286
3.7 5.29677142857143
3.8 4.62648648648649
3.9 4.113225
4 3.68651219512195
4.1 3.3197619047619
4.2 3.00602272727273
4.3 2.72302272727273
4.4 2.48247826086957
4.5 2.28476595744681
4.6 2.11242553191489
4.7 1.947875
4.8 1.79516666666667
4.9 1.63754
};
\addplot [semithick, black, mark=*, mark size=1, mark options={solid}]
table {%
1 10
1.1 10
1.2 10
1.3 10
1.4 10
1.5 10
1.6 10
1.7 10
1.8 10
1.9 10
2 10
2.1 10
2.2 10
2.3 10
2.4 10
2.5 10
2.6 10
2.7 10
2.8 9.999
2.9 9.994
3 9.948
3.1 9.757
3.2 9.053
3.3 7.749
3.4 6.125
3.5 4.94842857142857
3.6 4.10973913043478
3.7 3.52266666666667
3.8 3.06184
3.9 2.68708
4 2.39423076923077
4.1 2.15988461538462
4.2 1.98359259259259
4.3 1.82333333333333
4.4 1.63218518518519
4.5 1.43775
4.6 1.27560714285714
4.7 1.15134482758621
4.8 1.07882142857143
4.9 1.03565517241379
};
\addplot [semithick, gray, mark=*, mark size=1, mark options={solid}]
table {%
1 10
1.1 10
1.2 10
1.3 10
1.4 10
1.5 10
1.6 10
1.7 10
1.8 10
1.9 10
2 10
2.1 10
2.2 10
2.3 10
2.4 10
2.5 10
2.6 10
2.7 10
2.8 10
2.9 9.997
3 9.972
3.1 9.785
3.2 9.176
3.3 7.998
3.4 6.4435
3.5 5.29526086956522
3.6 4.45764285714286
3.7 3.87693181818182
3.8 3.41667391304348
3.9 3.06225531914894
4 2.7749375
4.1 2.51159183673469
4.2 2.30336
4.3 2.14192156862745
4.4 2.00772549019608
4.5 1.88717647058824
4.6 1.75171153846154
4.7 1.6051320754717
4.8 1.46509433962264
4.9 1.33998148148148
};
\addplot [semithick, black, dotted, mark=*, mark size=1, mark options={solid}]
table {%
1 10
1.1 10
1.2 10
1.3 10
1.4 10
1.5 10
1.6 10
1.7 10
1.8 10
1.9 10
2 10
2.1 10
2.2 10
2.3 10
2.4 10
2.5 10
2.6 10
2.7 9.988
2.8 9.906
2.9 9.559
3 8.455
3.1 7.046
3.2 5.5226
3.3 4.44018181818182
3.4 3.66792307692308
3.5 3.13103571428571
3.6 2.71879310344828
3.7 2.39429032258065
3.8 2.1409375
3.9 1.94312121212121
4 1.7505
4.1 1.54654285714286
4.2 1.34794594594595
4.3 1.204
4.4 1.10263157894737
4.5 1.04912820512821
4.6 1.01384615384615
4.7 0.98574358974359
4.8 0.949846153846154
4.9 0.88795
};


==> standalones/min_comp_uni_44_43_42_code_5/data.tex <==

\addplot [semithick, red!75.2941176470588!black, mark=square*, mark size=2.1, mark options={solid}]
table {%
1 0.0823769851601146
1.1 0.0798975527206457
1.2 0.0769755272064566
1.3 0.0744362145274668
1.4 0.0717361364228066
1.5 0.0689317885967196
1.6 0.0663434001562093
1.7 0.0634613381931789
1.8 0.0604820359281437
1.9 0.0578794584743556
2 0.0549067951054413
2.1 0.0520071595938558
2.2 0.0489367352252018
2.3 0.0457353553762041
2.4 0.0424860713355897
2.5 0.0390204373860974
2.6 0.0353302525384015
2.7 0.0312858630564957
2.8 0.0262101015360583
2.9 0.0198971621973444
3 0.011937646446238
3.1 0.00549804738349388
3.2 0.00148698255662588
3.3 0.000282962026258043
3.4 2.97130069186327e-05
3.5 2.23863722407947e-06
3.6 7.44724522620611e-08
};
\addlegendentry{4-bit MIM-H}
\addplot [semithick, red!75.2941176470588!black, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
1 0.0865620932048946
1.1 0.084107654256704
1.2 0.0812705024733142
1.3 0.0785429575631346
1.4 0.0759209841187191
1.5 0.0732302785732882
1.6 0.0706149440249935
1.7 0.0678643582400417
1.8 0.0647288466545171
1.9 0.0620689924498828
2 0.0591344701900547
2.1 0.0561568601926582
2.2 0.0530102837802656
2.3 0.0497650351470971
2.4 0.0466214527466806
2.5 0.0431455350169227
2.6 0.0393414475397032
2.7 0.0355415256443634
2.8 0.0309886748242645
2.9 0.0255579276230148
3 0.0179902369174694
3.1 0.0103208799791721
3.2 0.00379575631346004
3.3 0.000922112297144841
3.4 0.000138049986982557
3.5 1.11195001301744e-05
3.6 4.63754311475729e-07
};
\addlegendentry{3-bit MIM-H}
\addplot [semithick, red!75.2941176470588!black, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=x, mark size=3, mark options={solid}]
table {%
1 0.106031241864098
1.1 0.103683676126009
1.2 0.101380239520958
1.3 0.0989565217391304
1.4 0.0965338453527727
1.5 0.0938801093465243
1.6 0.091803306430617
1.7 0.0893016141629784
1.8 0.0863393647487633
1.9 0.0838659203332466
2 0.0812150481645405
2.1 0.0782724550898204
2.2 0.0756293933871388
2.3 0.0724614683676126
2.4 0.0695829211142932
2.5 0.0663439208539443
2.6 0.0627525384014579
2.7 0.0590812288466545
2.8 0.0552784431137725
2.9 0.0510554543087738
3 0.0457507159593856
3.1 0.0385006508721687
3.2 0.0280991929185108
3.3 0.0157606092163499
3.4 0.00574258005727675
3.5 0.00129438948190575
3.6 0.000190620932048946
3.7 1.32658129992349e-05
3.8 7.17572052000622e-07
};
\addlegendentry{2-bit MIM-H}
\addplot [semithick, color0, mark=square*, mark size=2.1, mark options={solid}]
table {%
1 0.0822344441551679
1.1 0.0796875813590211
1.2 0.0767022910700338
1.3 0.0741689664149961
1.4 0.0713394949231971
1.5 0.0684796927883364
1.6 0.0659321791200208
1.7 0.0629346524342619
1.8 0.0598598021348607
1.9 0.057133819317886
2 0.0540928143712575
2.1 0.0510687321010154
2.2 0.0479780005206977
2.3 0.0445639156469669
2.4 0.041396901848477
2.5 0.0377693309034106
2.6 0.0339815152304087
2.7 0.0299832074980474
2.8 0.0249164280135381
2.9 0.0187885967196043
3 0.0114178599323093
3.1 0.00516310856547774
3.2 0.00141278312939339
3.3 0.000278291243599757
3.4 2.72205295636694e-05
3.5 2.08244837556009e-06
3.6 9.27783986008448e-08
};
\addlegendentry{4-bit MIM-V}
\addplot [semithick, color0, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
1 0.0866059619890654
1.1 0.0841565998437907
1.2 0.0812206456651914
1.3 0.0786783389742255
1.4 0.0760096329080969
1.5 0.0731072637334028
1.6 0.0706787294975267
1.7 0.0677777922416038
1.8 0.0647045040354075
1.9 0.0620204373860974
2 0.059162978391044
2.1 0.0560545430877376
2.2 0.0531756053111169
2.3 0.0496120801874512
2.4 0.0467537099713616
2.5 0.0430842228586306
2.6 0.0394428534235876
2.7 0.0354095287685499
2.8 0.031092033324655
2.9 0.0255218693048685
3 0.0181386357719344
3.1 0.0102173913043478
3.2 0.00378378026555584
3.3 0.000998437906795105
3.4 0.000138505597500651
3.5 1.25322477574495e-05
3.6 5.46332084993892e-07
};
\addlegendentry{3-bit MIM-V}
\addplot [semithick, color0, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=x, mark size=3, mark options={solid}]
table {%
1 0.104336370736787
1.1 0.102054412913304
1.2 0.0995368393647488
1.3 0.0967475917729758
1.4 0.0943791981254882
1.5 0.0917046342098412
1.6 0.0890993230929445
1.7 0.0867167404321791
1.8 0.0837845613121583
1.9 0.0811060921634991
2 0.0785951575110648
2.1 0.0752737568341578
2.2 0.0724824264514449
2.3 0.0692572246810726
2.4 0.0662235095027337
2.5 0.0626681853683937
2.6 0.0590192658161937
2.7 0.0552215568862275
2.8 0.0512440770632648
2.9 0.0468738609737048
3 0.0414392085394429
3.1 0.0346789898463942
3.2 0.0249539182504556
3.3 0.0139047123145014
3.4 0.00518797188232231
3.5 0.00102564436344702
3.6 0.000161819838583702
3.7 1.23425917044629e-05
3.8 7.04731629618449e-07
};
\addlegendentry{2-bit MIM-V}
\addplot [very thick, black, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.0742491538661807
1.1 0.0716114293152825
1.2 0.0687003384535277
1.3 0.0661946107784431
1.4 0.0634448060400937
1.5 0.0605866961728716
1.6 0.058125748502994
1.7 0.0552973184066649
1.8 0.0522577453788076
1.9 0.0496959125227805
2 0.0468198385837022
2.1 0.0439902369174694
2.2 0.0412093204894559
2.3 0.0380997136162458
2.4 0.0353099453267378
2.5 0.0321972142671179
2.6 0.0291032283259568
2.7 0.0259006769070555
2.8 0.0225535016922676
2.9 0.0188027857328821
3 0.0142587867742775
3.1 0.00949049726633689
3.2 0.00452915907315803
3.3 0.00156983858370216
3.4 0.000293115632089858
3.5 3.16255361131284e-05
3.6 2.38469945505341e-06
3.7 8.2209560983097e-08
};
\addlegendentry{4-bit OMSQ-H}
\addplot [thick, gray, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.0742567039833377
1.1 0.0716165061181984
1.2 0.0686999479302265
1.3 0.0661936995574069
1.4 0.0634619890653476
1.5 0.060592033324655
1.6 0.0581210622233793
1.7 0.0553096849778703
1.8 0.0522442072376985
1.9 0.0497064566519136
2 0.0468272585264254
2.1 0.0440059880239521
2.2 0.0412425149700599
2.3 0.0381126008851862
2.4 0.0352854725331945
2.5 0.0321857589169487
2.6 0.0290472533194481
2.7 0.025874251497006
2.8 0.022526165061182
2.9 0.01875852642541
3 0.0142465503775059
3.1 0.00953670919031502
3.2 0.00461507419942723
3.3 0.00162880760218693
3.4 0.000310379241516966
3.5 3.37343216380538e-05
3.6 2.64043587383992e-06
3.7 9.82781665225254e-08
};
\addlegendentry{4-bit OMSQ-V}
\addplot [very thick, black, dotted, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.0711843530330643
1.1 0.0684462900286384
1.2 0.0657779484509242
1.3 0.0631647487633429
1.4 0.0605121322572247
1.5 0.0578193699557407
1.6 0.0550745899505337
1.7 0.0523721166362926
1.8 0.0495642280656079
1.9 0.0467935433480864
2 0.0439870085915126
2.1 0.0410789377766207
2.2 0.0381352252017704
2.3 0.0351269721426712
2.4 0.0319161155948972
2.5 0.0286027076282218
2.6 0.0251897292371778
2.7 0.021135837021609
2.8 0.0161532153085134
2.9 0.0103701417041693
3 0.0048585524602968
3.1 0.00163677782774372
3.2 0.000369095904301237
3.3 5.82220489592179e-05
3.4 7.31339253859431e-06
3.5 1.08318729906522e-06
3.6 2.24857123858653e-07
};
\addlegendentry{32-bit BP-H}
\addplot [thick, gray, dotted, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.0711843530330643
1.1 0.0684462900286384
1.2 0.0657779484509242
1.3 0.0631647487633429
1.4 0.0605121322572247
1.5 0.0578194220255142
1.6 0.0550746159854205
1.7 0.0523721166362926
1.8 0.0495642280656079
1.9 0.0467934392085394
2 0.0439869825566259
2.1 0.0410788076021869
2.2 0.0381359802134861
2.3 0.0351266857589169
2.4 0.0319159333506899
2.5 0.0286023171049206
2.6 0.0251917469409008
2.7 0.0211498090774972
2.8 0.0161860192658162
2.9 0.0104101610443709
3 0.00495762822181724
3.1 0.00169181202811768
3.2 0.000381379533423272
3.3 6.14614028658275e-05
3.4 7.72915241307072e-06
3.5 9.47865884966707e-07
};
\addlegendentry{32-bit BP-V}


==> tikz_prefs.tex <==
%auto-ignore
\usepackage{pgfplots}
\usepackage{tikz}

\usepackage{pgfplots}
\usepackage{tikzscale}
\usepackage{pgfkeys}
\pgfplotsset{compat=newest}
\pgfplotsset{every tick label/.append style={font=\footnotesize}}
\pgfplotsset{legend pos=outer north east}
\pgfkeys{
	/includetikzgraphic/.is family, /includetikzgraphic,
	default/.style = {
		width = \textwidth,
		ratio = 0.61803398875},
	width/.estore in = \itgWidth,
	ratio/.estore in = \itgRatio
}
\newlength\figurewidth
\newlength\figureheight
\newcommand{\includetikzgraphic}[2][]{
	\pgfkeys{/includetikzgraphic, default, #1}
	\setlength\figurewidth{\itgWidth}
	\setlength\figureheight{\itgRatio\figurewidth}
	\input{#2}
}


\usetikzlibrary{shapes,arrows,intersections,positioning,calc,automata,decorations.pathreplacing,decorations.markings, chains,fit,backgrounds, spy, matrix,decorations.pathreplacing}

\usepackage{tikzscale}
\usepackage{pgfkeys}
\pgfplotsset{compat=newest}
\pgfplotsset{every tick label/.append style={font=\footnotesize}}
\pgfplotsset{major grid style={solid, thin, gray}}
\pgfplotsset{minor grid style={solid, very thin, gray}}


\pgfplotsset{yticklabel style={text width=2.0em,align=right}}
\pgfplotsset{scale only axis=true}
\pgfplotsset{legend style={nodes={scale=0.7, transform shape}}}




